DiffPO: Diffusion-styled Preference Optimization for Efficient Inference-Time Alignment of Large Language Models

Inference-time alignment provides an efficient alternative for aligning LLMs with humans. However, these approaches still face challenges, such as limited scalability due to policy-specific value functions and latency during the inference phase. In this paper, we propose a novel approach, Diffusion-styled Preference Optimization (\model), which provides an efficient and policy-agnostic solution for aligning LLMs with humans. By directly performing alignment at sentence level, \model~avoids the time latency associated with token-level generation. Designed as a plug-and-play module, \model~can be seamlessly integrated with various base models to enhance their alignment. Extensive experiments on AlpacaEval 2, MT-bench, and HH-RLHF demonstrate that \model~achieves superior alignment performance across various settings, achieving a favorable trade-off between alignment quality and inference-time latency. Furthermore, \model~demonstrates model-agnostic scalability, significantly improving the performance of large models such as Llama-3-70B.

==> icml2025/sections/exp.tex <==
\section{Experiment}

\begin{table*}[t]
\caption{Performance of CoPO. It is shown that CoPO achieves significant performances in all the settings. When integrated and assessed in conjunction with various upstream models, the CoPO requires only a single training session (i.e., the CoPO model can operate in a zero-shot manner and enhance the performance of all upstream models.) The best result is highlighted in \textbf{bold}.}
\centering
\resizebox{0.98\textwidth}{!}{
  \begin{tabular}{l cccccccccc}
    \toprule
    \multirow{3}{*}{\textbf{Method}} & \multicolumn{5}{c}{Llama-3-SFT (8B)} & \multicolumn{5}{c}{Llama-3-Instruct (8B)} \\
    \cmidrule(r){2-6} \cmidrule(lr){7-11}
    &\multicolumn{1}{c}{MT-bench} & \multicolumn{2}{c}{AlpacaEval 2} &\multicolumn{2}{c}{HH-RLHF} & \multicolumn{1}{c}{MT-bench} & \multicolumn{2}{c}{AlpacaEval 2} &\multicolumn{2}{c}{HH-RLHF}\\
    \cmidrule(r){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-7}\cmidrule(lr){8-9} \cmidrule(lr){10-11}
           & GPT-4  & LC (\%) & WR (\%) & Helpful & Harmless & GPT-4  & LC (\%) & WR (\%) & Helpful & Harmless \\
    \hline
Base & 6.21 & 22.09 & 20.81 & 0.59 & 0.91 & 6.78 & 36.83 & 42.12 & 0.67 & 0.93 \\
DPO~\cite{rafailov2024direct} & 6.59 & 29.84 & 36.77 & 0.68 & 0.89 & 6.90 & 47.20 & 53.56 & 0.74 & 0.92 \\
SimPO~\cite{meng2024simposimplepreferenceoptimization} & 6.62 & 32.27 & 40.96 & 0.66 & 0.86 & 7.05 & 52.57 & 58.33 & 0.75 & 0.92 \\
BPO~\cite{cheng2024blackboxpromptoptimizationaligning} & 5.84 & 21.34 & 22.33 & 0.60 & 0.92 & 6.43 & 22.39 & 34.06 & 0.67 & 0.92 \\
ARGS~\cite{khanov2024argsalignmentrewardguidedsearch} & 6.14 & 9.06 & 13.97 & 0.49 & 0.86 & 6.84 & 31.83 & 34.74 & 0.64 & 0.89 \\
BoN~\cite{nakano2021webgpt} & 6.79 & 35.14 & 32.26 & 0.62 & 0.92 & 6.89 & 45.10 & 49.94 & 0.67 & 0.92 \\
Aligner~\cite{ji2024aligner} & 4.88 & 20.41 & 17.15 & 0.60 & 0.91 & 4.82 & 32.53 & 32.69 & 0.67 & 0.96 \\
MetaAligner~\cite{yang2024metaaligner} & 4.46 & 19.81 & 18.23 & 0.52 & 0.89 & 4.50 & 20.75 & 19.08 & 0.52 & 0.91 \\
CoPO & 6.96 & 36.24 & 40.96 & 0.62 & 0.93 & 6.88 & 35.51 & 40.28 & 0.67 & 0.93
\\\midrule
    \multirow{3}{*}{\textbf{Method}} & \multicolumn{5}{c}{Mistral-SFT (7B)} & \multicolumn{5}{c}{Mistral-Instruct (7B)} \\
    \cmidrule(r){2-6} \cmidrule(lr){7-11}
    &\multicolumn{1}{c}{MT-bench} & \multicolumn{2}{c}{AlpacaEval 2} &\multicolumn{2}{c}{HH-RLHF} & \multicolumn{1}{c}{MT-bench} & \multicolumn{2}{c}{AlpacaEval 2} &\multicolumn{2}{c}{HH-RLHF}\\
    \cmidrule(r){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-7}\cmidrule(lr){8-9} \cmidrule(lr){10-11}
           & GPT-4  & LC (\%) & WR (\%) & Helpful & Harmless & GPT-4  & LC (\%) & WR (\%) & Helpful & Harmless \\
\hline
Base & 5.73 & 20.15 & 17.24 & 0.56 & 0.87 & 6.39 & 32.81 & 34.86 & 0.66 & 0.94 \\
DPO~\cite{rafailov2024direct} & 5.91 & 31.28 & 32.65 & 0.66 & 0.91 & 6.29 & 35.60 & 37.73 & 0.67 & 0.92 \\
SimPO~\cite{meng2024simposimplepreferenceoptimization} & 6.17 & 31.16 & 33.72 & 0.63 & 0.86 & 6.36 & 35.78 & 40.21 & 0.67 & 0.93 \\
BPO~\cite{cheng2024blackboxpromptoptimizationaligning} & 5.55 & 18.23 & 17.23 & 0.64 & 0.92 & 5.99 & 19.61 & 27.49 & 0.66 & 0.93 \\
ARGS~\cite{khanov2024argsalignmentrewardguidedsearch} & 5.12 & 11.07 & 13.95 & 0.55 & 0.87 & 6.20 & 26.60 & 29.68 & 0.66 & 0.92 \\
BoN~\cite{nakano2021webgpt} & 6.21 & 33.36 & 27.74 & 0.64 & 0.94 & 6.40 & 34.75 & 39.24 & 0.68 & 0.94 \\
Aligner~\cite{ji2024aligner} & 4.27 & 18.27 & 15.53 & 0.60 & 0.95 & 4.42 & 28.88 & 30.30 & 0.66 & 0.93 \\
MetaAligner~\cite{yang2024metaaligner} & 4.08 & 12.40 & 9.72 & 0.51 & 0.85 & 3.71 & 18.55 & 16.91 & 0.55 & 0.91 \\
CoPO & 6.78 & 35.92 & 40.70 & 0.62 & 0.88 & 6.73 & 35.92 & 40.70 & 0.68 & 0.92 \\
\bottomrule
  \end{tabular}}
    \label{tab:methods_evaluation}
\end{table*}

\subsection{Experiment Setup}

\paragraph{Evaluation Datasets and Metrics.} 

We conduct our experiments using two widely adopted open-ended instruction-following benchmarks: \textit{MT-Bench} and \textit{AlpacaEval 2}. These benchmarks are designed to assess the models' conversational abilities over a varied set of queries. \textit{AlpacaEval 2} comprises 805 questions sourced from five distinct datasets, whereas \textit{MT-Bench} spans eight categories with a total of 80 questions.
We adhere to each benchmark's specific evaluation protocol for reporting scores. In the case of \textit{AlpacaEval 2}, we report both the raw win rate (WR) and the length-controlled win rate (LC) when compared against the GPT-4 model. For \textit{MT-Bench}, we present the average \textit{MT-Bench} score, utilizing GPT-4 as the judge model.
Furthermore, we utilize the \textit{HH-RLHF} datasets, which are instrumental in evaluating how well the models' generative capabilities align with human values, emphasizing helpfulness and harmlessness. Within the \textit{HH-RLHF} context, we report scores using \textit{ArmoRM}~\cite{ArmoRM}, a state-of-the-art reward model on \textit{RewardBench}, which reflects human preferences.

\paragraph{Baselines}
We compare \textbf{CoPO} with two main categories of offline preference optimization methods. In the \textbf{training phase}, \textit{Direct Preference Optimization (DPO)}~\cite{rafailov2024direct} reparameterizes reward functions to simplify and stabilize the preference learning process. \textit{SimPO}~\cite{meng2024simposimplepreferenceoptimization}, on the other hand, uses the average log probability of a sequence as an implicit reward, aligning more closely with model generation.
In the \textbf{inference phase}, \textit{Black-Box Prompt Optimization (BPO)}~\cite{cheng2024blackboxpromptoptimizationaligning} adapts user prompts to better align with LLMs' input comprehension, thereby optimally achieving user intents without altering LLM parameters. \textit{ARGS}~\cite{khanov2024argsalignmentrewardguidedsearch} integrates alignment into the decoding process via reward-guided search, removing the need for costly RL training. Finally, \textit{Best-of-N sampling (BoN)}~\cite{nakano2021webgpt} samples N times and selects the highest-scoring sample based on the reward model. In our experiments, we use \textit{ArmoRM}~\cite{ArmoRM} as the reward model and set N to 4. \textit{Aligner}~\cite{ji2024aligner} and \textit{MetaAligner}~\cite{yang2024metaaligner} employ an additional model to learn corrective residuals between preferred and dispreferred responses to refine model generation.


\paragraph{Base Models and Inference Settings.} We perform preference optimization using two model families, \textit{Llama-3-8B} and \textit{Mistral-7B}, under two configurations: SFT and Instruct. For the SFT configuration, we employ open-source models by \textit{SimPO} following \textit{Zephyr}, training a base model (i.e., \texttt{mistralai/Mistral-7B-v0.1} or \texttt{meta-llama/Meta-Llama-3-8B}) on the \textit{UltraChat-200k} dataset to derive an SFT model. For the Instruct configuration, we utilize an off-the-shelf instruction-tuned model.

During the inference phase, we initially generate basic responses from the base models. For \textit{AlpacaEval 2} and \textit{HH-RLHF}, we utilize a sampling decoding strategy with a temperature setting of 0.7. For \textit{MT-Bench}, we follow the official decoding configuration, which prescribes varying temperatures across different categories. In all experiments, the maximum length of new tokens is primarily set to 256. Subsequently, we apply the trained \textit{CoPO} model to these basic responses, maintaining a sentence length of 256.

\subsection{Experiment Results}

\paragraph{CoPO significantly outperforms existing preference optimization methods.} As shown in Table~\ref{tab:methods_evaluation}, while all preference optimization algorithms enhance performance over the SFT model, CoPO, achieves the best overall performance across all benchmarks and settings. These consistent and significant improvements highlight the robustness and effectiveness of CoPO. 
%Notably, CoPO outperforms the best baseline by 3.6 to 4.8 points on the AlpacaEval 2 LC win rate across various settings. On Arena-Hard, CoPO consistently achieves superior performance,

\paragraph{CoPO consistently improves the performance of base models of various sizes.}




\begin{table*}[t]
\caption{Comparison of baseline methods and CoPO. The best result is highlighted in \textbf{bold}.}
\centering
\resizebox{0.85\textwidth}{!}{
  \begin{tabular}{cc cccccccc}
    \toprule
    \multirow{2}{*}{\textbf{CoPO Models}} & \multirow{2}{*}{\textbf{Models}} 
    &\multicolumn{3}{c}{MT-bench} & \multicolumn{2}{c}{AlpacaEval 2} &\multicolumn{3}{c}{HH-RLHF} \\
    \cmidrule(r){3-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} 
           && GPT-4 & Turbo & Turbo & LC (\%) & WR (\%) & Armo & Armo & Armo  \\
    \hline
CoPO-2B  & Llama-3.2-1B-Instruct & 
\\\bottomrule
  \end{tabular}}
    \label{tab:methods_evaluation}
\end{table*}

\begin{figure}[h] % 'h' here means to place the figure here, near the text
    \centering
    \label{fig: performance_vs_time}
    \includegraphics[width=0.5\textwidth]{icml2025/figs/performance_vs_time.pdf} % Adjusts the size of the image to 50% of the text width
    \caption{\textbf{Comparison of Inference-Time Compute Efficiency.} We compare CoPO with existing inference-time alignment techniques based on both alignment performance and execution time across three datasets. Points located closer to the top-right corner indicate a more favorable Pareto frontier. To facilitate effective presentation, we applied min-max normalization to both performance and execution time metrics.}
\end{figure}

\paragraph{CoPO achieves surpassing Inference-Time Efficiency.}

\subsection{Analysis}

==> icml2025/sections/intro.tex <==
\section{Introduction}

The alignment of large language models (LLMs) with human preferences has recently emerged as a focal area of research \cite{wang2023aligning, shen2023large}. Prominent techniques such as Reinforcement Learning from Human Feedback (RLHF) \cite{ouyang2022training} and Direct Preference Optimization (DPO) \cite{rafailov2024direct} have demonstrated substantial efficacy in aligning models with human values. However, these methods require the optimization of individual policies, which presents challenges such as high consumption of training resources. 
Inference-time alignment \cite{mudgal2023controlled, han2024value} provides an efficient alternative by directly adjusting the model's output distribution, thus avoiding the need for resource-intensive retraining. Despite its advantages, this approach still requires policy-specific value functions, limiting its scalability across different models. Additionally, the inference-time latency remain prohibitively high, presenting further challenges to its practical deployment.


%In parallel, recent developments highlight the potential of Diffusion Language Models (DLMs) for controllable, any-order, and parallel text generation, as evidenced by Venkatraman et al. (2024) and Gong et al. (2023a). Notably, DLMs show promising capabilities for intermediate token correction (Ye et al., 2024) and global planning (Zhang et al., 2023), which address significant limitations inherent in the autoregressive (AR) approach.
\begin{figure*}[h] % 'h' here means to place the figure here, near the text
    \centering
    \includegraphics[width=\textwidth]{icml2025/figs/framework.png}
    \caption{\textbf{Illustration of the \model~Framework.} (a) The objective of LLM alignment is to adjust the output of LLMs to align with human values and intentions. In this process, preferences are defined at the \textbf{sentence level}, focusing on the style and format of the complete output. (b) We propose Diffusion-style Preference Optimization (\model), which reconceptualize alignment process as a sentence-level denoising process, where the goal is to progressive predict aligned sentence $\by^{(T)}$ from unaligned sentence $\by^{(0)}$. In the training stage, \model~model $\pi_\theta$ is trained to consistently transform any unaligned output of the base LLM into an aligned response.
    (c) As a plug-and-play module, optimized \model~can be directly intergrated with the output of the base model and enhance its alignment level.}
    \label{fig: illustration}
\end{figure*}

In this paper, we investigate to develop an efficient and policy-agnostic preference alignment method.
We first reconsider the objective of \textit{align} with humans~\cite{yao2023instructions, shen2023large}, as illustrated in Fig.~\ref{fig: illustration}(a).
The alignment is on sentence-level, requires steering only the key component of generated content, such as style or format, to meet human intentions or reflect human values. 
Drawing inspiration from the global controllability of diffusion models~\cite{li2022diffusion,lyu2023fine}, we propose Diffusion-styled Preference Optimization (\model), which reconceptualizes the alignment as a diffusion-styled denoising process.

By employing parallel decoding~\cite{santilli2023accelerating, leviathan2023fast}, \model~directly predicts transition between sentences. 
we define the process of alignment as ``next-sentence prediction.''
Our approach begins with the text generated by an unaligned model. By employing parallel decoding of autoregressive models, the alignment process progressively predicts the next sentence towards human preference, ultimately forecasting an aligned generation.
% the alignment process modeling of Large Language Models (LLMs). Drawing inspiration from the Superficial Alignment Hypothesis, we posit that alignment could be a straightforward process where the model learns the style or format for interacting with users, leveraging the knowledge and capabilities already acquired during pre-training. 
Our goal is to train an LLM that can predict more aligned outputs based on any unaligned generation. Building upon the concepts of Consistency Models~\cite{song2023consistency} and Consistency LLMs~\cite{kou2024cllms}, we propose Consistency Preference Optimization, a novel approach that agnostically aligns different unaligned outputs. By defining the transition from an unaligned generation to an aligned generation for the same prompt as a trajectory, we employ an objective that maps any intermediate generations with varying degrees of alignment on the Jacobi trajectory to the aligned generation. In this way, a notable property of our model is self-consistency: it maps sentences on the same trajectory to a more preferred sentence. 


% Imagining the evolution of the n-token sequence as the denoising process of a natural image (Ho et al., 2020; Song et al., 2021b), we surprisingly find that the above learning procedure draws a sharp analogy to the acceleration technique for diffusion models named consistency models (CMs)

% 我们发现与RLHF的目标一致性


Extensive analysis shows that \model~utilizes preference data more effectively, leading to a more accurate likelihood ranking of winning and losing responses on a held-out validation set, which in turn translates to a better policy model. As shown in Table 1, our method achieves state-of-the-art performance, with a 72.4\% length-controlled win rate on AlpacaEval 2 and a 59.1\% win rate on Arena-Hard, establishing it as the strongest open-source model under 10B parameters. Most notably, when evaluated on Chatbot Arena [17] with real user votes, our model significantly improved upon the initial model, advancing from 36th to 25th place and ranking first among all $<$10B models on the leaderboard.

\sj{I think you should rephrase the contribution as twofold: 1) we are more resource-efficient than SIMPO and DPO. 2) we are complimentary to them as we are inference time aligner and show DPO/SIMPO+\model results.}



==> icml2025/sections/method.tex <==
\section{Method}

\subsection{Preliminaries}

\paragraph{The Objective of Large Language Models Alignment.}
The standard text generation process of large language models (LLMs) with prompt $\bx$ and response $\by$ can be defined as a token-level Markov Decision Process (MDP). 
MDP is denoted as a tuple $\mathcal{M} = (\mathcal{S}, \mathcal{A}, \mathcal{P}, R, T)$, where the state space $\mathcal{S}$ consists of the prompt and all tokens generated so far (i.e., $\bs_t= (\bx, \by_{1:t-1})$). The action space $\mathcal{A}$ is the tokens from the vocabulary (i.e., $\ba_t = \by_{t}$). $\mathcal{P}$ is the transition kernel, which is deterministic that given state $\bs_t= (\bx, \by_{1:t-1})$ and action $\ba_t = \by^{(t)}$, the next state is $\bs_{t+1}= (\bs_{t}, \ba_t)= (\bx, \by_{1:t})$. R : $\mathcal{S} \times \mathcal{A} \to \mathbb{R}$ represents the reward at each step. The maximum token count, $T$, sets the length limit for LLM outputs, which conclude with an end-of-sentence (EoS) token $\by_{t}=$ EoS that ends the generation. 
The language model is a (Markov) policy $\pi : \mathcal{S} \to \Delta(\mathcal{A})$ that maps from state to a distribution over actions.

During the alignment of LLMs, the objective is to optimize a language model $\pi_\theta$ that maximizes the reward, where the reward reflects user's preference.
\begin{equation}
\label{RLHF_objective}
\max_{\pi_\theta} \mathbb{E}_{\substack{x \sim D, y \sim \pi_\theta(y|x)\\y' \sim \pi_{\text{ref}}(y|x)} } \left[ p(y \succ y' | x) - \beta D_{KL}(\pi_\theta \| \pi_{\text{ref}}) \right],
\end{equation}
where \( p(y \succ y' | x) \) represents the human preference, i.e., the probability that \( y \) is preferred over \( y' \) given the context \( x \), which can be represented by the general reward function \( R \) in traditional RLHF framework. The parameter \( \beta \) controls the deviation from the base reference policy \( \pi_{\text{ref}} \), which corresponds to the initial Supervised Fine-Tuning (SFT) model \( \pi_{\text{SFT}} \).


% \paragraph{Existing LLM Alignment Techniques.}

\paragraph{Parallel Decoding of LLMs}
Given a prompt $x$ and a pre-trained LLM $\pi(\cdot|x)$, the model response is typically obtained with the standard AR decoding method under the greedy strategy, i.e.,
\begin{equation}
y_i = \arg\max_y \pi(y|y_{<i}, x) \quad \text{for } i = 1, \ldots, n 
\end{equation}
where $y_{<i}$ denotes $\{y_1, \ldots, y_{i-1}\}$. As shown, $n$ forward passes of the LLM are required to obtain $n$ tokens $y_{\leq n}$. 

In comparison, parallel decoding has demonstrated the capacity to reduce the inference costs of LLMs by enabling sentence-level generation and improving content quality. Concretely, supposing
\begin{equation}
f(y_i, y_{<i}, x) := y_i - \arg\max_y \pi(y|y_{<i}, x),
\end{equation}
parallel decoding re-frames the LLM inference process as solving a system of nonlinear equations w.r.t. $y_i$:
\begin{equation}
f(y_i, y_{<i}, x) = 0 \quad \text{for } i = 1, \ldots, n.
\end{equation}
It can be solved in parallel:
\begin{equation}
\left\{
\begin{aligned}
y_1^{(j+1)} &= \arg \max_y \pi(y \mid x) \\
y_2^{(j+1)} &= \arg \max_y \pi(y \mid y_1^{(j)}, x) \\
& \vdots \\
y_n^{(j+1)} &= \arg \max_y \pi(y \mid y_{<n}^{(j)}, x)
\end{aligned}
\right.
\end{equation}
In this way, for one forward pass of the LLM, we can obtain the next sentence $y^{(j+1)}$ based on the previous one $y^{(j)}$.

\sj{The connection between Jacobi decoding and alignment is not clear.}
\rz{My point here is that Sec 2.2 combine them together}

\subsection{Alignment as Next-Sentence Prediction}
\paragraph{Motivation.}
Inspired by the multifaceted goals of LLM alignment, which include adhering to human instructions, conforming to human intentions, and reflecting broader human values \cite{yao2023instructions}, we observe a distinct pattern in the alignment process. Unlike pre-training phases that focus on acquiring capabilities such as text generation, alignment specifically aims to modify the style or format of generation to better suit interactions with users. This prompts us to reconsider how to ``order'' the alignment process.
% Inspired by the goals of LLM alignment, which involve adhering to human instructions, conforming to human intentions, and reflecting broader human values~\cite{yao2023instructions}, we observe a distinct aspect of this alignment process. Unlike pre-training phases that focus on acquiring knowledge, alignment involves training the model to learn the style or format necessary for interacting with users. This perspective aligns with the views presented in the Superficial Alignment Hypothesis \cite{zhou2024lima}.
% As inspired by the goals of LLM alignment, which involve varying levels of alignment goals including adhering to human instructions, conforming to human intentions, and reflecting human values~\cite{yao2023instructions}. Superficial Alignment Hypothesis~\cite{zhou2024lima} also posits that alignment is a process where the model learns the style or format for interacting with users, leveraging the knowledge already acquired during pre-training. 
\sj{The motivation is unclear.}
\sj{Need a figure in intro motivate readers.} \rz{Yes. Will include a figure.}

\paragraph{Reformulation.} We propose to reconceptualize alignment as a straightforward process of ``Next-Sentence Prediction,'' wherein the alignment process is envisioned as the continuous prediction of sentences that progressively align with human values, thereby holistically adjusting the format, style, and values of the generated content. The Next-Sentence Prediction is formulated as: \sj{Are we sticking to the true notion of sentence here? next sentence prediction in this paper can easily be confused with Bert's next sentence prediction. I think we better just write this as a diffusion process e.g., diffusion path prediction.} \rz{Yea, I will rethink that}
\begin{equation}
p(y^{(T)}) := p(y^{(0)}) \prod_{t=1}^T p(y^{(t)} \mid y^{(t-1)}, x),
\end{equation}
% Inspired by \cite{12}, we draw an analogy between the alignment of Large Language Models (LLMs) and a denoising process. In this context, ``denoising'' does not refer to the traditional removal of noise from signals but rather to the reduction of undesirable biases and errors in the model's outputs, thereby aligning them more closely with human preferences.
where we denote the initial unaligned generation and the aligned generation as $y^{(0)}$ and $y^{(T)}$, respectively. The sequence $y^{(1:T-1)}$ can be understood as the intermediate unaligned generations that are distributed along the trajectory from $y^{(0)}$ to $y^{(T)}$.


% The goal of alignment is to output the preferred \( y^{(0)} \) by denoising \( y^{(t)} \): \( p_\theta(y^{0:T}) := p(y^{(t)}) \prod_{t=1}^T p_\theta(y^{t-1} \mid y^{(t)}) \), a discrete-time reverse process with a Markov structure.
% \sj{I am confused by the notations here. you need equation 7 in terms of x?}
% \rz{Yesterday haven't finished the writing start from here. Sorry for the confusion. I have revised following equations and notations now.}

Here, we assume there exists a reward model $R(x, y)$ which reflects the alignment of the generation $y$ for input $x$ with human preferences. Therefore, our aim can be formulated to learn a function $p_\theta(y^{(t)} \mid y^{(t-1)})$ that produces paths $(y^{(0)}, y^{(1)}, \dots, y^{(T)})$ that ultimately result in a high-reward (aligned) generation $y^{(T)}$. Each transition can be viewed as:
\begin{align}
p_\theta(y^{(t)} \mid y^{(t-1)}, x) \propto p(y^{(t)} \mid y^{(t-1)}, x)\text{exp}(R(x, y^{(t)})).
\end{align}
\sj{Yes, I think diffusion path prediction sounds better than next sentence prediction.}
% Specifically, we use a transformer architecture to model \( f_\theta \), which spontaneously models the semantic relation between \( x_t \) and \( y^{(t)} \). We compute the variational lower bound (\( \mathcal{L}_{\text{VLB}} \)) following the original diffusion process.
% \begin{align}
% \mathcal{L}_{\text{VLB}} =& \mathbb{E}_{p_\theta(y^{(t)} \mid y^{(t-1)})} R(x, y^{(t)}).
% \end{align}


\subsection{Consistency Preference Optimization (CoPO)}

We propose Consistency Preference Optimization (CoPO), a sentence-level optimization strategy that improves the alignment of generations with human preferences. Inspired by Consistency Models~\cite{song2023consistency} and Consistency LLMs~\cite{kou2024cllms}, we propose to consistently map any intermediate generation $y^{(t)}$ to the aligned generation $y^{(T)}$.
We jointly optimize two losses, one aligning the intermediate generation with the aligned generation and the other avoiding the model from deviating from the base LLM so as to maintain generation quality.

\textbf{Consistency Loss.} For a prompt \( x \) with an unaligned generation $y^{(t)}$, we directly push the model to output $y^{(T)}$ with $y^{(t)}$ as the input by minimizing the following loss:
\begin{align}
\label{gc_loss}
L_{\text{Con}} = \mathbb{E}_{(x, y^{(t)}, y^{(T)}) \sim \mathcal{D}} \left[ \sum_{i=1}^n \text{KL}(p_{\theta^-} (y_{<i}^{(T)}, x) \| p_\theta (y_{<i}^{(t)}, x)) \right],
\end{align} 
where \(\theta^- = \text{stopgrad}(\theta)\) and $n$ denotes the length of generation. \( \text{KL}(\cdot \| \cdot) \) denotes the forward KL distance between two distributions. \sj{What is n in eq 8? i assume it is the generation length right?} \rz{Yes, added explanation } \sj{Why stopgrad?}\rz{because both the two terms calls $p_\theta$, I guess it prevents collapse in optimization like in SimSiam \url{https://arxiv.org/pdf/2011.10566}}

\textbf{AR Loss.} To avoid deviating from the distribution of the base LLM, we incorporate the traditional AR loss based on the generation \( y^{(T)} \) of the base LLM \( p \):
\begin{align}
L_{\text{AR}} = \mathbb{E}_{(x,y^{(T)}) \sim \mathcal{D}} \left[ -\sum_{i=1}^N \log p_\theta(y^{(T)}_i | y^{(T)}_{<i}, x) \right]
\end{align}
This term contributes to maintaining the generation quality.
Consequently, the total loss for CoPO is:
\begin{align}
\label{total_loss}
L(\theta) = L_{\text{Con}} + \omega L_{\text{AR}},
\end{align}
where \( \omega \) represents a weighting coefficient.

\subsection{The Objective of CoPO within RLHF Framework}

In this section, we analyze the role of CoPO in the goal of RLHF. 
We start with the same RL objective as prior work, Eq.~\ref{RLHF_objective}, under a general reward function r. Following prior work [31, 30, 19, 15], it is straightforward to show that the optimal solution to the KL-constrained reward maximization objective in Eq. 3 takes the form:
\begin{equation}
r^*(x, y) = \beta \log \left( \frac{\pi^*(y \mid x)}{\pi_{\text{ref}}(y \mid x)} \right) + \beta \log Z(x).
\end{equation}
where \( Z(x) = \sum_y \pi_{\text{ref}}(y | x) \exp\left( \frac{1}{\beta} r^*(x, y) \right) \) is the partition function. With Bradley-Terry model, we can represent the preference function as the difference of rewards:
\begin{align}
    p(y \succ y' | x) &= \sigma(r^*(x, y) - r^*(x, y')) \\
    &= \sigma \left( \log \frac{\pi^*(y \mid x)}{\pi_{\text{ref}}(y \mid x)}  - \log \frac{\pi^*(y' \mid x)}{\pi_{\text{ref}}(y' \mid x)} \right)
\end{align}
Substitute $\pi^*(y \mid x)$ with $\pi_{\text{CoPO}}(y \mid y',x)\pi_{\text{ref}}(y' \mid x)$:
% \begin{align}
%     p(y \succ y' | x) 
%     &= \sigma \left( \log \frac{\pi_{CoPO}(y \mid y',x)\pi_{\text{ref}}(y' \mid x)}{\pi_{\text{ref}}(y \mid x)}  - \log \frac{\pi_{CoPO}(y' \mid y',x)\pi_{\text{ref}}(y' \mid x)}{\pi_{\text{ref}}(y' \mid x)} \right)\\
%     &= \sigma \left( \log \frac{\pi_{CoPO}(y \mid y',x)\pi_{\text{ref}}(y' \mid x)}{\pi_{\text{ref}}(y \mid x)}  - \log \pi_{CoPO}(y' \mid y',x) \right)\\
%     &= \sigma \left( \log \frac{\pi_{CoPO}(y \mid y',x)}{\pi_{CoPO}(y' \mid y',x)}  - \log \frac{\pi_{\text{ref}}(y' \mid x)}{\pi_{\text{ref}}(y \mid x)} \right)
% \end{align}
\begin{align}
\label{eq:copo}
    p(y \succ y' | x) 
    &= \sigma \left( \log \frac{\pi_{\text{CoPO}}(y \mid y',x)}{\pi_{\text{CoPO}}(y' \mid y',x)}  - \log \frac{\pi_{\text{ref}}(y' \mid x)}{\pi_{\text{ref}}(y \mid x)} \right),
\end{align}
where the first term in Eq.~\ref{eq:copo} is optimized by the consistency loss in Eq.~\ref{gc_loss}, while the second term in Eq.~\ref{eq:copo} remains constant. 
In summary, the objective of CoPO in Eq.~\ref{total_loss} is consistent with the RLHF objective in Eq.~\ref{RLHF_objective}.





% We consider the general objective for RLHF, based on maximizing a non-linear function of preferences. To this end, we consider a general non-decreasing function \( \Psi : [0, 1] \to \mathbb{R} \), a reference policy \( \pi_{\text{ref}} \in \Delta \mathcal{Y} \), and a real positive regularisation parameter \( \tau \in \mathbb{R}^+ \), and define the \( \Psi \)-preference optimisation objective (\( \Psi\text{PO} \)) as
% \[
% \max_\pi \mathbb{E}_{x \sim \rho, y \sim \pi(\cdot|x), y' \sim \mu(\cdot|x)} \left[ \Psi(p^*(y \succ y' | x)) \right] - \tau D_{\text{KL}}(\pi \| \pi_{\text{ref}}), 
% \]
% where the human preference $p^*(y \succ y' | x)$ the probability of y being preferred to y knowing the context x.
% This objective balances the maximisation of a potentially non-linear function of preference probabilities with the KL regularisation term which encourages policies to be close to the reference \( \pi_{\text{ref}} \). This objective strictly generalises both RLHF and DPO, when the BT model holds.








\subsection{Practical Implementations}

\paragraph{Generate Intermediate Generations.}

To realize CoPO, we collect a set of intermediate generations on each prompt, forming an original training set $\mathcal{D}$. Specifically, we use prompts from the UltraFeedback dataset~\cite{cui2023ultrafeedback}. For each prompt $x$, we generate 6 responses using 6 base models. We then use ArmoRM~\cite{ArmoRM} to score the 6 responses, selecting the highest-scoring one as $y^{(T)}$. The other five responses are ranked according to their scores to serve as $y^{(0:T-1)}$.


\paragraph{Training and Inference.} In the training phase, we initialize our aligning model $p_\theta$ with Llama-3-8B-Instruct and optimize it using CoPO. Note that since the lengths of the intermediate generations in $\mathcal{D}$ vary, we employ padding or truncation to standardize their lengths. Then, in the inference phase, we employ the optimized model $p_\theta^*$ to align the responses of vanilla generations from different models. 


\paragraph{Discussion.}
To summarize, the advantages of CoPO can be summarized as follows:
\begin{enumerate}
    \item \textbf{Model-agnostic:} CoPO is trained with the objective of consistently predicting sentences with better alignment quality, allowing it to be applied to various base LLMs. This enables us to train a single model for a given preference without the need to align all base LLMs. Moreover, the CoPO model does not require parameter access, making it also suitable for API-based models.
    \item \textbf{Training and Inference Efficient:} As a post-inference alignment strategy, CoPO avoids the need for resource-intensive alignment of numerous models and instead requires training only an additional small model to achieve alignment. Furthermore, by modeling as next-sentence prediction, the model can predict better sentences during each forward pass, optimizing the trade-off between alignment methods and inference speed during the inference phase.
\end{enumerate}


\subsection{Connection to Consistency Models}
The development of CoPO is mainly inspired by Consistency Models~\cite{song2023consistency} and CLLMs~\cite{kou2024cllms}. Consistency models address the limitation of the slow iterative sampling process by mapping any point along the probability flow ODE of the diffusion process back to the original point in a single step. CLLMs propose accelerating LLM inference by mapping the intermediate process of LLM parallel decoding to the final process. Similar to these works, we draw an analogy between the generation of LLMs and a denoising process. However, we view ``denoising'' as the reduction of undesirable biases and errors in the model's outputs, thereby employing a different objective, aligning them more closely with human preferences.





==> icml2025/sections/method2.tex <==
\section{Method}

\subsection{Preliminaries: Large Language Models}

\paragraph{Next-Token Prediction.}
The text generation of autoregressive large language models (LLMs) with prompt $\bx$ and response $\by$ can be modelled as a next-token prediction process. Given a sequence of input tokens $\bx = (\bx_1, \bx_2, . . . , \bx_m)$, 
The language model is a policy $\pi(\cdot|x)$ that autoregressively maps from current tokens $(\bx, \by_{1:n-1})$ to a distribution over the next token $\by_n$.
The maximum token count, $N$, sets the length limit for LLM outputs, which conclude with an end-of-sentence (EoS) token $\by_{n}=$ EoS that ends the generation. The generated output $\by$ consists of predicted tokens $(\by_1, \by_2, . . . , \by_N)$.

\paragraph{The Objective of Alignment.}
During the alignment of LLMs, the objective is to optimize a language model $\pi_\theta$ that maximizes the user's preference~\cite{christiano2017deep, ouyang2022training,rafailov2024direct}:
\begin{align}
\label{RLHF_objective}
\max_{\pi_\theta} \mathbb{E}_{\substack{x \sim D, \by \sim \pi_\theta(\by|\bx)\\\by' \sim \pi_{\mathrm{ref}}(\by|\bx)} }& [ p(\by \succ \by' | \bx) \nonumber\\&- \beta D_{KL}(\pi_\theta \| \pi_{\mathrm{ref}}) ],
\end{align}
where \( p(\by \succ \by' | \bx) \) represents the preference, i.e., the probability that \( \by \) is preferred over \( \by' \) given the context \( \bx \), which can be generally represented by the reward function \( R \) in traditional RLHF framework. The parameter \( \beta \) controls the deviation from the base reference policy \( \pi_{\mathrm{ref}} \), which corresponds to the Supervised Fine-Tuning (SFT) model.
The human preference \( p(\by \succ \by' | \bx) \) is defined at the sentence level, which evaluates the holistic performance of the entire response \( \by \). However, due to the next-token prediction modeling in LLMs, existing alignment techniques must optimize the preference (reward) at the token level, complicating the learning process~\cite{andrychowicz2017hindsight, zhong2024dpo, zeng2024token}.

% \paragraph{Existing LLM Alignment Techniques.}

\paragraph{Parallel Decoding of LLMs}

In comparison to next-token prediction, where token-level generation is performed sequentially to obtain a sentence, parallel decoding has demonstrated the capacity by enabling sentence-level generation and improving content quality~\cite{santilli2023accelerating, leviathan2023fast}. Concretely, supposing
\begin{equation}
f(\by_n, \by_{<n}, \bx) := \by_n - \arg \max_\by \pi(\by|\by_{<n}, \bx), \nonumber
\end{equation}
parallel decoding re-frames the LLM inference process as solving a system of nonlinear equations w.r.t. $\by_n$:
\begin{equation}
f(\by_n, \by_{<n}, \bx) = 0 \quad \text{for time } t = 1, \ldots, T. \nonumber
\end{equation}
It can be solved in a parallel and iterative way bt Jacobi decoding:
\begin{equation}
\left\{
\begin{aligned}
\by_1^{(t+1)} &= \arg \max_\by \pi(\by \mid \bx) \\
\by_2^{(t+1)} &= \arg \max_\by \pi(\by \mid \by_1^{(t)}, \bx) \\
& \vdots \\
\by_N^{(t+1)} &= \arg \max_\by \pi(\by \mid \by_{<N}^{(t)}, \bx)
\end{aligned}
\right.
\end{equation}
In this way, for one forward pass of the LLM, we can obtain the next sentence $\by^{(t+1)}$ based on the previous one $\by^{(t)}$.

\subsection{Diffusion-styled Preference Optimization}

\paragraph{Motivation.}
The goal of LLM alignment is to align the generation of LLMs with human values or intentions~\cite{yao2023instructions}. In this process, preferences are defined at the \textbf{sentence-level}, focusing on the style or format of complete answers generated by the LLMs, as illustrated in Fig.~\ref{fig: illustration}(a). However, the generation of these responses occurs at the token level, following the next-token prediction pattern inherent in LLM modeling. This requires existing alignment techniques to optimize preferences (or rewards) at the \textbf{token-level}. This inconsistency prompts us to reconsider the formulation of the alignment process.

% Inspired by the multifaceted goals of LLM alignment, which include adhering to human instructions, conforming to human intentions, and reflecting broader human values \cite{yao2023instructions}, we observe a distinct pattern in the alignment process. Unlike pre-training phases that focus on acquiring capabilities such as text generation, alignment specifically aims to modify the style or format of generation to better suit interactions with users. 

% Inspired by the goals of LLM alignment, which involve adhering to human instructions, conforming to human intentions, and reflecting broader human values~\cite{yao2023instructions}, we observe a distinct aspect of this alignment process. Unlike pre-training phases that focus on acquiring knowledge, alignment involves training the model to learn the style or format necessary for interacting with users. This perspective aligns with the views presented in the Superficial Alignment Hypothesis \cite{zhou2024lima}.
% As inspired by the goals of LLM alignment, which involve varying levels of alignment goals including adhering to human instructions, conforming to human intentions, and reflecting human values~\cite{yao2023instructions}. Superficial Alignment Hypothesis~\cite{zhou2024lima} also posits that alignment is a process where the model learns the style or format for interacting with users, leveraging the knowledge already acquired during pre-training. 
% \sj{The motivation is unclear.}
% \sj{Need a figure in intro motivate readers.} \rz{Yes. Will include a figure.}

\paragraph{Reformulation.} 
Inspired by the potential benefits of diffusion process in controllable sentence generation~\cite{gong2022diffuseq,han2022ssd,ye2024diffusion}, we draw an analogy between the alignment of LLMs and the diffusion process.
We propose Diffusion-styled Preference Optimization (\model), which reconceptualize alignment process as a sentence-level denoising process.
The denoising process gradually align the original output $\by^{(T)}$ from $\by^{(0)}$ by learning a denoising model $\pi_\theta$, thereby holistically adjusting the format, style, and values of the generated content, as illustrated in Fig.~\ref{fig: illustration}(b). The sentence-level alignment process is formulated as:
% We propose to reconceptualize alignment as a straightforward process of ``Next-Sentence Prediction,'' wherein the alignment process is envisioned as the continuous prediction of sentences that progressively align with human values, thereby holistically adjusting the format, style, and values of the generated content, as illustrated in Fig.~\ref{fig: illustration}(b). The Next-Sentence Prediction is formulated as: \sj{Are we sticking to the true notion of sentence here? next sentence prediction in this paper can easily be confused with Bert's next sentence prediction. I think we better just write this as a diffusion process e.g., diffusion path prediction.} \rz{Yea, I will rethink that}
\begin{equation}
\pi_\theta(\by^{(0:T)}) := p(\by^{(0)}) \prod_{t=1}^T \pi_\theta(\by^{(t)} | \by^{(t-1)}, \bx),
\end{equation}
% Inspired by \cite{12}, we draw an analogy between the alignment of Large Language Models (LLMs) and a denoising process. In this context, ``denoising'' does not refer to the traditional removal of noise from signals but rather to the reduction of undesirable biases and errors in the model's outputs, thereby aligning them more closely with human preferences.
where we denote the initial unaligned generation and the aligned generation as $\by^{(0)}$ and $\by^{(T)}$, respectively. The sequence $\by^{(1:T-1)}$ can be understood as the intermediate unaligned generations that are distributed along the trajectory from $\by^{(0)}$ to $\by^{(T)}$.
% The goal of alignment is to output the preferred \( y^{(0)} \) by denoising \( y^{(t)} \): \( p_\theta(y^{0:T}) := p(y^{(t)}) \prod_{t=1}^T p_\theta(y^{t-1} \mid y^{(t)}) \), a discrete-time reverse process with a Markov structure.
% \sj{I am confused by the notations here. you need equation 7 in terms of x?}
% \rz{Yesterday haven't finished the writing start from here. Sorry for the confusion. I have revised following equations and notations now.}
Assume there exists a reward model $R(\bx, \by)$ which reflects the alignment of the generation $\by$ given input $\bx$ with human preferences. Therefore, the aim of alignment can be formulated to learn a function $\pi_\theta(\by^{(t)} | \by^{(t-1)})$ that produces a trajectory $(\by^{(0)}, \by^{(1)}, \dots, \by^{(T)})$ that ultimately result in a high-reward (aligned) generation $\by^{(T)}$. Each transition can be viewed as:
\begin{align}
\pi_\theta(\by^{(t)} | \by^{(t-1)}, \bx) \propto p(\by^{(t-1)}, \bx){\text{exp}}(R(\bx, \by^{(t)})). \nonumber
\end{align}
% \sj{Yes, I think diffusion path prediction sounds better than next sentence prediction.}
% Specifically, we use a transformer architecture to model \( f_\theta \), which spontaneously models the semantic relation between \( x_t \) and \( y^{(t)} \). We compute the variational lower bound (\( \mathcal{L}_{\text{VLB}} \)) following the original diffusion process.
% \begin{align}
% \mathcal{L}_{\text{VLB}} =& \mathbb{E}_{p_\theta(y^{(t)} \mid y^{(t-1)})} R(x, y^{(t)}).
% \end{align}


\subsection{Consistency Optimization of \model}

Inspired by Consistency Models~\cite{song2023consistency} and Consistency LLMs~\cite{kou2024cllms}, we propose to consistently map any intermediate generation $\by^{(t)}$ to the aligned generation $\by^{(T)}$.
We jointly optimize the \model~model $\pi_\theta$ with two losses, one aligning the intermediate generation with the aligned generation and the other avoiding the model from deviating from the base LLM so as to maintain generation quality.

\textbf{Consistency Loss.} For a prompt \( \bx \) with an unaligned generation $\by^{(t)}$, we directly push the model to output $\by^{(T)}$ with $\by^{(t)}$ as the input by minimizing the following loss $L_{\mathrm{Con}}$=
\begin{align}
\label{gc_loss}
\mathbb{E}_{(\bx, \by^{(t)}, \by^{(T)}) \sim \mathcal{D}} \left[ \sum_{i=1}^N \mathrm{KL}(\pi_{\theta^-} (\by_{<i}^{(T)}, \bx) \| \pi_\theta (\by_{<i}^{(t)}, \bx)) \right]
\end{align} 
where \(\theta^- = \mathrm{stopgrad}(\theta)\) and $N$ denotes the length of generation. \( \mathrm{KL}(\cdot \| \cdot) \) denotes the forward KL distance between two distributions. 

\textbf{AR Loss.} To avoid deviating from the distribution of the base LLM, we incorporate the traditional AR loss based on the generation \( \by^{(T)} \) of the base LLM \( \pi_{\mathrm{ref}} \):
\begin{align}
L_{\mathrm{AR}} = \mathbb{E}_{(\bx,\by^{(T)}) \sim \mathcal{D}} \left[ -\sum_{i=1}^N \log \pi_\theta(\by^{(T)}_i | \by^{(T)}_{<i}, \bx) \right].
\end{align}
This term contributes to maintaining the generation quality.
Consequently, the total loss for~\model~is:
\begin{align}
\label{total_loss}
L(\theta) = L_{\mathrm{Con}} + \omega L_{\mathrm{AR}},
\end{align}
where \( \omega \) represents a weighting coefficient. \sj{I do not see any ablation show $L_Con$ is actually helpful. One may argue that just having a model trained to predict aligned from unaligned would be enough.}

\subsection{The Objective of \model~within RLHF Framework}

In this section, we analyze the role of \model~in the goal of RLHF. 
We start with the same RL objective as prior work, Eq.~\ref{RLHF_objective}, under a general reward function r. Following prior work~\cite{peng2019advantage, rafailov2024direct}, it is straightforward to show that the optimal solution to the KL-constrained reward maximization objective in Eq. 3 takes the form:
\begin{equation}
r^*(\bx, \by) = \beta \log \left( \frac{\pi^*(\by \mid \bx)}{\pi_{\mathrm{ref}}(\by \mid \bx)} \right) + \beta \log Z(\bx).
\end{equation}
where \( Z(\bx) = \sum_\by \pi_{\mathrm{ref}}(\by | \bx) \exp\left( \frac{1}{\beta} r^*(\bx, \by) \right) \) is the partition function. With Bradley-Terry model, we can represent the preference function as the difference of rewards: 
%\sj{I am sorry but the notations must need to improve. Use $y_w$ and $y_l$ instead to denote winner and loser as we are talking about preference optimization.}
\begin{align*}
    p&(\by_w \succ \by_l | \bx) = \sigma(r^*(\bx, \by_w) - r^*(\bx, \by_l)) \\
    &= \sigma \left(\beta  \log \frac{\pi^*(\by_w \mid \bx)}{\pi_{\mathrm{ref}}(\by_w \mid \bx)}  -\beta  \log \frac{\pi^*(\by_l \mid \bx)}{\pi_{\mathrm{ref}}(\by_l \mid \bx)} \right).
\end{align*}
Substitute by $\pi^*(\by \mid \bx)= \pi_{\mathrm{\model}}(\by \mid \by',x)$ $\pi_{\mathrm{ref}}(\by' \mid \bx)$, we have $p(\by_w \succ \by_l | \bx)$
\begin{align}
\label{eq:parpo}
    =\sigma \left( \beta \log \frac{\pi_{\mathrm{\model}}(\by_w \mid \by_l,\bx)}{\pi_{\mathrm{\model}}(\by_l \mid \by_l,\bx)}  - \beta \log \frac{\pi_{\mathrm{ref}}(\by_w \mid \bx)}{\pi_{\mathrm{ref}}(\by_l \mid \bx)} \right).
\end{align}
\sj{I am a little confused here. What does ${\pi_{\mathrm{\model}}(y' \mid y',x)}$ indicate?} \rz{It can be understood combining with Eq. 7, where we maximize the probability of predicting $y_w$ compared with $y_l$.}
Note that the first term in Eq.~\ref{eq:parpo} is optimized through the consistency loss in Eq.~\ref{gc_loss}, while the second term in Eq.~\ref{eq:parpo} depends only on $\bx$, with the base policy $\pi_{\mathrm{ref}}$ held constant. Moreover, the deviation from the base policy can be easily controlled, as $\by_w$ is derived from $\by_l$.

\textit{In summary, the objective of \model~as defined in Eq.~\ref{total_loss} aligns with the RLHF objective in Eq.~\ref{RLHF_objective}.} Furthermore, since \( \pi_{\text{\model}} \) is optimized independently from the reference model \( \pi_{\text{ref}} \) to ensure alignment, it can be deployed in a model-agnostic manner.
 
%\sj{Is $y'$ generated from $y$? I thought it was the other way around.}





% We consider the general objective for RLHF, based on maximizing a non-linear function of preferences. To this end, we consider a general non-decreasing function \( \Psi : [0, 1] \to \mathbb{R} \), a reference policy \( \pi_{\text{ref}} \in \Delta \mathcal{Y} \), and a real positive regularisation parameter \( \tau \in \mathbb{R}^+ \), and define the \( \Psi \)-preference optimisation objective (\( \Psi\text{PO} \)) as
% \[
% \max_\pi \mathbb{E}_{x \sim \rho, y \sim \pi(\cdot|x), y' \sim \mu(\cdot|x)} \left[ \Psi(p^*(y \succ y' | x)) \right] - \tau D_{\text{KL}}(\pi \| \pi_{\text{ref}}), 
% \]
% where the human preference $p^*(y \succ y' | x)$ the probability of y being preferred to y knowing the context x.
% This objective balances the maximisation of a potentially non-linear function of preference probabilities with the KL regularisation term which encourages policies to be close to the reference \( \pi_{\text{ref}} \). This objective strictly generalises both RLHF and DPO, when the BT model holds.


\subsection{Practical Implementations}

\paragraph{Generate Intermediate Generations.}

To implement \model, we collect a set of intermediate generations on each prompt, forming an original training set $\mathcal{D}$. Specifically, we use prompts from the UltraFeedback dataset~\cite{cui2023ultrafeedback}. For each prompt $\bx$, we generate 6 responses using 6 base models. We then use ArmoRM~\cite{ArmoRM} to score the 6 responses, selecting the highest-scoring one as $\by^{(T)}$. The other five responses are ranked according to their scores to serve as $\by^{(0:T-1)}$.


\paragraph{Training and Inference.} In the training phase, we initialize our aligning model $\pi_\theta$ with Llama-3-8B-Instruct and optimize it using \model. Note that since the lengths of the intermediate generations in $\mathcal{D}$ vary, we employ padding or truncation to standardize their lengths. Then, in the inference phase, we employ the optimized model $\pi_\theta^*$ to align the responses of vanilla generations from different models. 


\paragraph{Discussion.}
To summarize, the advantages of \model~can be summarized as follows:
\begin{enumerate}
    \item \textbf{Model-agnostic:} \model~is trained with the objective of consistently predicting sentences with better alignment quality, allowing it to be applied to various base LLMs. This enables us to train a single model for a given preference without the need to align all base LLMs. Moreover, the \model~model does not require parameter access, making it also suitable for API-based models. \sj{Why don't we align some of the latest models like GPT4o, Deepseek-V3 etc.? These experiments will really help the paper.}
    \item \textbf{Training and Inference Efficient:} As a post-inference alignment strategy, \model~avoids the need for resource-intensive alignment of numerous models and instead requires training only an additional small model to achieve alignment. \sj{Perhaps this is not so correct to claim? when we use a 9B model to align a 7B model, I do not think we can call ourselves resource-efficient.} Furthermore, by modeling as next-sentence prediction, the model can predict better sentences during each forward pass, optimizing the trade-off between alignment methods and inference speed during the inference phase. \sj{sorry, this is unclear. need to explain with notations.}
    \item \sj{Can use on top of existing preference aligned models.}
\end{enumerate}








==> icml2025/sections/related_works.tex <==
\section{Related Works}

\paragraph{Align LLM with Human Preference.}

A prominent approach to learning from human preferences is RLHF \cite{ouyang2022training, stiennon2020learning, christiano2017deep, bai2022training}. In this framework, a reward model is first trained, followed by the training of a bandit policy using Proximal Policy Optimization (PPO) \cite{schulman2017proximal}. 
Recent advancements such as direct preference optimization (DPO) \cite{rafailov2024direct, meng2024simposimplepreferenceoptimization, ethayarajh2024kto} optimize the bandit policy directly from human preferences, bypassing the need for a reward model. These approaches are simpler to implement and require fewer computational resources.
Inference-time approaches, on the other hand, achieve alignment by customizing the output of large language models (LLMs) during the decoding phase, without the need for parameter optimization. This results in enhanced flexibility and efficiency~\cite{khanov2024argsalignmentrewardguidedsearch, mudgal2023controlled}. One representative method treats the text-generation process as a search problem, guided by external rewards \cite{huang2024deal, han2024value, chakraborty2024transfer}. Another category of methods focuses on learning to refine the generated text~\cite{li2023rain, ji2024aligner, yang2024metaaligner}.

\paragraph{Token and Sentence-level.}
Existing training-based or inference-time alignment approaches typically rely on token-level rewards, while human preferences are generally provided and defined at the sentence level \cite{li2023remax, ahmadian2024back, zeng2024token}. To address this discrepancy, some works \cite{lightman2023let, yang2024preference, zeng2024token} leverage token-wise or step-wise information to improve alignment performance. 
In contrast, this paper proposes modeling alignment as a sentence-level denoising process. We introduce a model-agnostic, inference-time alignment method, and our empirical results demonstrate its superiority in both performance and efficiency. Additional related works can be referred to in Appendix~\ref{appendix: related works}.
